Equational reasoning with context-free families of string diagrams

String diagrams provide an intuitive language for expressing networks of interacting processes graphically. A discrete representation of string diagrams, called string graphs, allows for mechanised equational reasoning by double-pushout rewriting. However, one often wishes to express not just single equations, but entire families of equations between diagrams of arbitrary size. To do this we define a class of context-free grammars, called B-ESG grammars, that are suitable for defining entire families of string graphs, and crucially, of string graph rewrite rules. We show that the language-membership and match-enumeration problems are decidable for these grammars, and hence that there is an algorithm for rewriting string graphs according to B-ESG rewrite patterns. We also show that it is possible to reason at the level of grammars by providing a simple method for transforming a grammar by string graph rewriting, and showing admissibility of the induced B-ESG rewrite pattern.

==> background.tex <==
% -*- root: main.tex -*-

% \subsection{String Graphs}

% In this work, the central objects of study are special kinds of graphs, called
% \textit{String Graphs}. 
% String Graphs were originally introduced under the name "Open Graphs" in
% \cite{open_graphs}, \cite{open_graphs1}. Since then, the theory has been
% further developed and the term was changed to "String Graphs" in
% \cite{kissinger_dphil}. String graphs were introduced in order to represent
% String Diagrams in a way that allows efficient automation by computer systems.
% String diagrams were in turn intrdouced by Roger Penrose in
% \cite{penrose_tensor} as a way to conviniently represent Abstract Tensor
% Systems. 

% String graphs are a special kind of typed directed graphs. Every vertex of a
% string graph is either a wire-vertex or a node-vertex. Node-vertices should be
% thought of as the main vertices of the graph, whereas wire vertices are only
% there to assist with technicalities related to rewriting of string graphs.
% An important notion regarding string graphs is wire-homeomorphism. Two string
% graphs are wire-homeomorphic if we can get one from the other by increasing and
% decreasing the number of wire vertices on certain wires. Semantically,
% wire-homeomorphic string graphs are considered to be equal. As an example, the
% following two graphs are wire-homeomorphic:




% For reasons of simplicity and brevity, in this paper we assume that all node vertices are of the same type, all wire vertices are also of the same type and all edges also share the same type.  These assumptions are convenient, but not necessary. All of our grammatical constructions can easily accommodate different types on vertices and edges, unless otherwise noted. For this reason, the definitions we provide for string graphs and !-graphs are simpler compared to the ones given in other works, because we can simply ignore some of the
% typing constraints.
% Next, we provide definitions for string graphs and related notions.


%\subsection{!-graphs}

\begin{definition}[Graph \cite{graph_grammar_handbook}]
  A \textit{graph} over an alphabet of node labels $\Sigma$ and an alphabet of edge
  labels $\Gamma$ is a tuple $H = (V, E, \lambda)$, where $V$ is a finite set
  of nodes, $E \subseteq \{(v, \gamma, w) | v, w \in V, v \not= w, \gamma \in
  \Gamma\}$ is the set of edges and $\lambda : V \to \Sigma$ is the node
  labelling function. The set of all graphs with labels $\Sigma, \Gamma$ is denoted $GR_{\Sigma,\Gamma}$.
\end{definition}

\begin{remark}
Note, that this definition of graphs does not allow for self-loops. This is a standard (and convenient) assumption in the C-edNCE literature. By using this notion of graphs, we do not lose any expressivity for string graphs, because any string graph with a self-loop is wire-homeomorphic (see Definition~\ref{def:wire-homeo}) to a string graph with no self-loops.
\end{remark}

\begin{definition}[String Graph] \label{def:string-graph}
  A \textit{string graph} is a graph labelled by the set $\{ N, W \}$, where vertices labelled $N$ are called \textit{node-vertices} and vertices labelled $W$ are called \textit{wire-vertices}, and the following conditions hold:
  (1) there are no edges directly connecting two node-vertices,
  (2) the in-degree of every wire-vertex is at most one and
  (3) the out-degree of every wire-vertex is at most one.
\end{definition}

We will depict wire vertices as small black dots and node-vertices as larger white circles, as we have already done in Section~\ref{sec:intro}.
  For simplicity, we assume there is only one type of node-vertex, but we could easily capture string graphs like~\ref{fig:string-diagram-encode} by taking the labels to be $\{ N_f, N_g, N_h, W \}$, for example.

We also identify those wire-vertices which form the boundary of a string graph:

\begin{definition}[Inputs, Outputs and Boundary Vertices]
A wire-vertex of a string graph $G$ is called an \textit{input} if it has no incoming
edges. A wire-vertex with no outging edges is called an \textit{output}. We denote
with $\textit{In}(G)$ and $\textit{Out}(G)$ the string graphs with no edges whose
vertices are respectively the inputs and outputs of $G$. The boundary of
$G$ is $\textit{Bound}(G) := \textit{In}(G) \cup \textit{Out}(G)$.
\end{definition}

Just as node-vertices represent the boxes in a string diagram, chains of wire-vertices represent the wires. 

\begin{definition}[Wires]
  A connected chain of vertices where each endpoint is either a boundary or a node-vertex, and all other vertices are wire-vertices is called a \textit{closed wire}. A closed wire minus its endpoints is called the \textit{interior} of a closed wire. A cycle consisting only of wire-vertices is called a \textit{circle}.
\end{definition}

Often, it is more natural to consider an equivalence class of string graphs, up to \textit{wire homeomorphism}.


% Next, we provide some definitions which make the notion of wire-homeomorphism precise.

% \begin{definition}[Simple Chains and Cycles]
%   A \textit{simple chain} is a connected, acyclic graph where each vertex has
%   at most one in-edge and one out-edge. A vertex in a chain with only an
%   in-edge or only an out-edge is called an $endpoint$. A \textit{simple cycle}
%   is a connected graph where each vertex has exactly one in-edge and one
%   out-edge.
% \end{definition}

% \begin{definition}[Closed Wire]
%   For a string graph $H$, a \textit{closed wire} $W \subseteq G$ is a simple
%   cycle of wire vertices or a simple chain such that:
%   \begin{enumerate}
%     \item the endpoints of $W$ are either node-vertices or in the boundary of
%       $G$ and
%     \item all other vertices in $W$ are wire-vertices.
%   \end{enumerate}
% \end{definition}

% \begin{definition}[Homeomorphpic wires]
%   Two wires $W$ and $W'$ are said to be \textit{homeomorphic} if they are both circles
% \end{definition}

\begin{definition}[Wire-homeomorphic string graphs] \label{def:wire-homeo}
  Two string graphs $G$ and $G'$ are called \textit{wire-homeomorphic}, written $G \sim G'$ if $G'$ can be obtained from $G$ by either merging two adjacent wire-vertices (left) or by splitting a wire-vertex into two adjacent wire-vertices (right) any number of times:
    \[ \stikz[0.7]{two-wires.tikz} \ \ \mapsto \ \ \stikz[0.7]{one-wire.tikz}
      \quad\quad\quad\quad
    \stikz[0.7]{one-wire.tikz} \ \ \mapsto \ \ \stikz[0.7]{two-wires.tikz} \]
\end{definition}

\begin{wrapfigure}{R}{0.4\textwidth}
  \centering
  \stikz[0.6]{wire-homeo.tikz}
  \caption{Wire homeomorphism}\label{fig:homeo}
\end{wrapfigure}
That is, two graphs are wire-homeomorphic if the only difference between them is the number of wire-vertices used to represent a wire in the diagram
(see Fig.\ref{fig:homeo}).

% !-graphs (pronounced \textit{bang graphs}) were introduced in
% \cite{pattern_graphs} under the name \textit{pattern graphs} and were later
% renamed to their current name in \cite{merry_dphil} which contains the most
% complete and detailed description of !-graphs.

% A !-graph is a generalised string graph which allows us to represent infinite
% families of string graphs in a formal way. In addition to wire and box
% vertices, !-graphs also have a third type of vertices, called !-vertices. The
% edges coming out of a !-vertex determine a !-box whose contents can be copied
% infinitely many times (while preserving connection relations), thus allowing us
% to represent an infinite set of string graphs in a finite way.

% The motivation behind !-graphs is to remove some of the informalities in
% expressing infinite families of rewrite rules and infinite families of diagrams
% using the familiar "dot dot dot" $(\cdots)$ notation in order to ease the
% development of software proof-assistants.

Next, we provide definitions for !-graphs and related notions. First, we need to identify which subgraphs are legal to put in !-boxes.

\begin{definition}[Open Subgraph]
  A subgraph $O$ of a string graph $H$ is said to be \textit{open} if it is a full subgraph and furthermore $\textit{In}(H \backslash
  O) \subseteq \textit{In}(H)$ and $\textit{Out}(H \backslash O) \subseteq \textit{Out}(H)$.
\end{definition}


\begin{definition}[!-graph]
  A \textit{!-graph} $H$ is a string graph, a partially ordered set $!(H)$ of \textit{!-boxes}, and an open subgraph $B(b) \subseteq H$ for every $b \in !(H)$ such that $b \leq b' \implies B(b) \subseteq B(b')$.
\end{definition}

The notion of openness ensures that we never put only part of a wire inside a !-box, which would cause wires to ``split'' in the middle as we expand the !-box, which violates the arity conditions for wire-vertices from Definition~\ref{def:string-graph}.

% \cstikz[0.7]{split-ends.tikz}


If $b_2 \leq b_1$, this means that $b_2$ is \textit{nested} inside of $b_1$, which we indicate by drawing a line connecting their corners. This is to distinguish from the case where $b_1$ and $b_2$ merely \textit{overlap}.
\[
\stikz[0.7]{bang_graph-nest.tikz}
\qquad\qquad\textrm{vs}\qquad\qquad
\stikz[0.7]{bang_graph-overlap.tikz}
\]


\begin{definition}[Concrete Graph]
A !-graph with no !-vertices is called a \textit{concrete
graph} or simply a string graph.
\end{definition}

% \begin{example}
% We draw !-vertices as blue box-shaped nodes and all their outgoing edges are
% colored in blue. Wire and box vertices are drawn as before (as a small black
% dot and white circle respectively).
% \cstikz[0.7]{bang_graph1.tikz}
% The above depiction of a !-graph is a little cluttered, so instead of drawing
% the edges associated with a !-vertex, we will simply draw a blue box around
% all the nodes which are adjacent to it (hence the name !-box). Like so:
% \cstikz[0.7]{bang_graph2.tikz}
% \end{example}

A !-graph represents an infinite set of concrete string graphs, each of which is obtained after a finite number of applications of the EXPAND and KILL operations presented below.

\begin{definition}[!-box Operations]
The two primitive !-box operations are as follows:
% For a !-graph $G$ and a !-vertex $b \in G$, the three !-box operations are
% functions which produce a new !-graph as follows:
\begin{itemize}
  \item $\textrm{KILL}_b(G) = G' \backslash B(b)$
  \item $\textrm{EXPAND}_b(G) = G \ \sqcup_{KILL_b(G)}\  G'$
\end{itemize}
where $G'$ has the same underlying string graph as $G$, but with $b$ and all of its children removed from $!(G)$. The expression for EXPAND is the disjoint union of $G$ and $G'$, with the vertices, edges, and !-boxes in the common subgraph $\textrm{KILL}_b(G)$ identified.
\end{definition}

As seen in~\eqref{eq:bbox-ops}, $\textrm{KILL}_b$ removes a !-box $b$ and its contents, whereas $\textrm{EXPAND}_b$ inserts a new copy of the contents of $b$. See~\cite{pattern_graphs} for a more detailed description of these operations.

% where $succ(b)$ is the set of all successors of the !-vertex $b$ (which
% includes itself) and the copy operation is the quotient of the disjoint union
% of $G$ with itself over the KILL operation applied to the same !-box.

% In other words, applying a DROP operation removes a !-box, but not its
% contents:
% \cstikz[0.7]{drop.tikz}
% applying a KILL operation removes a !-box and its contents:
% \cstikz[0.7]{kill.tikz}
% applying a COPY operation creates another copy of the !-box and its contents
% which is connected in the same way to the rest of the graph:
% \cstikz[0.7]{tikz/copy.tikz}

% Semantically, a !-graph represents the infinite set of concrete string graphs
% obtained after applying all possible sequences of !-box operations.

\begin{definition}[!-graph Language]
  The \textit{language} of a !-graph $G$ is the set of all concrete string graphs obtained by applying a sequence of !-box operations on $G$.
\end{definition}

% \begin{example}
% The language of the running example is given by:

% \cstikz[0.7]{tikz/bang_graph_semantics.tikz}
% \end{example}

Note that overlapping !-boxes are not explicitly ruled out. However, they can create some odd non-local behaviour. So, na\"ively, one might want to rule out overlap entirely, but it turns out that certain instances of overlap are more innocent than others.

% These we call \textit{trivially overlapping}.

% Finally, we provide definitions which fully characterize the possible
% relationships between a pair of !-boxes $b_1$ and $b_2$.

\begin{definition}[Overlap and Trivial Overlap]
  Given a pair of non-nested !-boxes $b_1$ and $b_2$, we say that $b_1$ and $b_2$ are \textit{overlapping} if $B(b_1) \cap B(b_2) \not = \emptyset$.
  %and otherwise we say that they are \textit{disjoint}.
  $b_1$ and $b_2$ \textit{overlap trivially} if $B(b_1) \cap B(b_2)$ consists of only the interior of zero or more closed wires, where one endpoint is a node-vertex only in $B(b_1)$ and the other is a node-vertex only in $B(b_2)$.
\end{definition}

\begin{wrapfigure}{r}{0.4\textwidth}
\centering
\stikz[0.65]{bang_relationship.tikz}
\caption{Trivial vs non-trivial overlap}\label{fig:bb_overlap}
\end{wrapfigure}
In particular, $B(b_1) \cap B(b_2)$ can be empty, so trivial overlap generalises no-overlap. In Fig.~\ref{fig:bb_overlap} $b_1$ and $b_2$ overlap trivially, since they only overlap on the interior of a wire connecting node-vertices in the two boxes. $b_3$ and $b_4$ overlap non-trivially, since they overlap on a node-vertex. The most subtle case is $b_5$ and $b_6$, which overlap non-trivially because the shared wire-vertices are not part of a wire whose endpoints are in distinct !-boxes. Of course, all other pairs of !-boxes overlap trivially, as their intersection is just the empty set.

\begin{definition}[\textbf{BGTO}]
  A !-graph where any two non-nested !-boxes overlap trivially is called a \textit{!-graph with trivial overlap}. The set of all languages induced by these !-graphs is called \textbf{BGTO}.
\end{definition}

%\subsection{Vertex replacement grammars}
\input{graph_grammars.tex}


==> graph_grammars.tex <==
Next, we introduce C-edNCE graph grammars. Graph grammars are a generalization of context-free grammars for strings. A graph grammar consists of a finite collection of productions which specify instructions on how to generate a family of graphs. Like their context-free string counterparts, context-free graph grammars have better structural, decidability and complexity properties compared to other more expressive mechanisms for graph transformation. We use the same definitions and conventions for graph grammars as presented in \cite{graph_grammar_handbook}, which also describes C-edNCE grammars and their properties in much greater detail.

% \begin{definition}[Graph Language \cite{graph_grammar_handbook}]
%   The set of all graphs over $\Sigma$ and $\Gamma$ is denoted by $GR_{\Sigma,
%   \Gamma}$. The set of all graphs modulo graph isomorphism is denoted by
%   $[GR_{\Sigma, \Gamma}]$. A \textit{graph language} is a subset of
%   $[GR_{\Sigma, \Gamma}]$.
% \end{definition}

C-edNCE grammars are built using graphs with embedding. These provide the information needed to replace a non-terminal node with a new graph, and update connections accordingly.

\begin{definition}[Graph with embedding \cite{graph_grammar_handbook}]
  A \textit{Graph with embedding} over labels $\Sigma, \Gamma$ is a pair $(H,
  C),$ where $H$ is a graph over $\Sigma, \Gamma$ and $C \subseteq \Sigma
  \times \Gamma \times \Gamma \times V_H \times \{in, out\}$. $C$ is called a \textit{connection relation} and its elements are called \textit{connection instructions}. The set of all graphs with embedding over $\Sigma, \Gamma$ is denoted by $GRE_{\Sigma, \Gamma}$.
\end{definition}

Graph grammars operate by substituting a graph (with embedding) for a non-terminal node of another graph. Connection instructions are used to introduce edges connected to the new graph based on edges connected to the non-terminal. A connection instruction as $(\sigma, \beta / \gamma, x, d)$ says to add an edge labelled $\gamma$ connected to the vertex $x$ in the new graph, for every $\beta$-labelled edge connecting a $\sigma$-labelled vertex to the non-terminal. $d$ then indicates whether this rule applies to in-edges or out-edges of the non-terminal. More formally:

\begin{definition}[Graph Substitution \cite{graph_grammar_handbook}]
  Let $(H, C_H), (D, C_D) \in GRE_{\Sigma,\Gamma}$ be two graphs with
  embedding, where $H$ and $D$ are disjoint. Let $v \in V_H$ be a node of $H$.
  The \textit{substitution} of $(D, C_D)$ for $v$ in $(H, C_H)$ is denoted by
  $(H, C_H)[v/(D,C_D)]$ and is given by the graph with embedding whose
  components are:
  \begin{align*}
    V \quad=\quad &(V_H - \{v\} )\cup V_D\\
    E \quad=\quad &\{(x,\gamma,y)\in E_H | x \not = v, y\not = v\} \cup E_D\\
    &\cup \{(w,\gamma,x)\ |\ \exists \beta \in \Gamma : (w,\beta,v) \in E_H
      ,(\lambda_H(w), \beta / \gamma, x,in)\in C_D \}\\
    &\cup \{(x,\gamma,w)\ |\ \exists \beta \in \Gamma : (v,\beta,w) \in E_H
      ,(\lambda_H(w), \beta / \gamma, x,out)\in C_D \}\\
    \lambda(x) \quad=\quad
      &\begin{cases}
	\lambda_H(x) & \text{if } x \in (V_H - \{v\})\\
	\lambda_D(x) & \text{if } x \in V_D
      \end{cases}\\
    C \quad=\quad &\{(\sigma,\beta / \gamma,x,d) \in C_H\ |\ x \not = v\}\\
    &\cup \{(\sigma,\beta / \delta,x,d)\ |\ \exists \gamma \in \Gamma :
    (\sigma,\beta / \gamma,v,d) \in C_H,(\sigma, \gamma / \delta,x,d)\in C_D\}
  \end{align*}
\end{definition}

Thankfully, graphs with embedding allow for a simple graphical presentation (see Fig.~\ref{fig:subst}). We draw graphs as in the previous sections, but with the additional convention that nodes with non-terminal labels are drawn as boxes instead of circles. A single connection instruction is drawn as a pair of edges crossing the outer frame. The edge and node types outside of the frame specify neighbouring node(s) which are connected to the non-terminal in the host graph and the edge(s) inside the frame indicate what new edges will be constructed to and from those nodes.

% We can think of a graph with embedding as just a normal graph with some
% additional information which describes how the graph should be embedded into
% another graph while performing the productions of a graph grammar. In
% particular, a connection instruction $(\sigma, \beta/ \gamma,x,in)$ for a graph
% with embedding $(H, C)$ means that for every $\sigma$ labelled node $w$ in the
% mother graph for which there is a $\beta$ labeled edge going \textbf{in}to the
% non-terminal node $v$ of the mother graph which is being replaced, then the
% embedding process will establish a $\gamma$ labeled edge from $w$ to $x$. This
% should become more clear after referring to fig. \ref{fig:subst} which provides
% an example of graph substitution. The meaning for $(\sigma, \beta/
% \gamma,x,out)$ is analogous.

% If a graph with embedding has no connection instructions (i.e. $C=\emptyset$), then we can think of it as just an ordinary graph.

% Fig.~\ref{fig:subst} shows an example of graph substitution,
% where the newly established edges are colored in red.
  \begin{figure}
    \cstikz[0.6]{tikz/subst_example1.tikz}
    \caption{
      \textbf{(1)} Graph with embedding $(H,C_H)$
      \textbf{(2)} Graph with embedding $(D,C_D)$
      \textbf{(3)} Result of substitution $(H,C_H)[v/(D,C_D)]$ where $v$ is
        the vertex with non-terminal label in $H$.}\label{fig:subst}
  \end{figure}

Next, we define the concept of an edNCE Graph Grammar. edNCE is an
abbreviation for \textbf{N}eighbourhood \textbf{C}ontrolled \textbf{E}mbedding
for \textbf{d}irected graphs with dynamic \textbf{e}dge relabeling. 

\begin{definition}[edNCE Graph Grammar \cite{graph_grammar_handbook}]
  An \textit{edNCE Graph Grammar} is a tuple $G = (\Sigma, \Delta, \Gamma,
  \Omega, P, S)$, where 
    $\Sigma$ is the alphabet of node labels,
    $\Delta \subseteq \Sigma$ is the alphabet of terminal node labels,
    $\Gamma$ is the alphabet of edge labels,
    $\Omega \subseteq \Gamma$ is the alphabet of final edge labels,
    $P$ is a finite set of productions and
    $S \in \Sigma - \Delta$ is the initial nonterminal.
  Productions are of the form $X \rightarrow (D, C)$, where $X \in \Sigma -
  \Delta$ is a non-terminal node and $(D, C) \in GRE_{\Sigma, \Gamma}$ is a
  graph with embedding.
\end{definition}
  We can graphically depict an edNCE grammar by depicting all of its
  productions. A production is drawn exactly like a graph with embedding
  with the addition that we depict its associated non-terminal in the top-left
  part of the frame.
\begin{example}\label{ex:line_graph}
  The following grammar generates the set of all chains of node vertices with an input and no outputs:
  \cstikz[0.7]{unbounded.tikz}
\end{example}

\begin{definition}[Derivation Step \cite{graph_grammar_handbook}]
  For a graph grammar $G=(\Sigma,\Delta,\Gamma,\Omega,P,S)$ and graphs (with
  embedding) $H, H' \in GRE_{\Sigma,\Gamma}$ consider a vertex $v \in V_H$
  and an isomorphic copy $p: X\to(D,C)$ of some production $p' \in P$. We say
  $H \Rightarrow_{v,p} H'$ is a \textit{derivation step} if $\lambda_H(v) = X$ 
  and $H'=H[v/(D,C)]$. If $v$ and $p$ are clear from the context, then we
  write $H \Rightarrow H'$. A sequence of derivation steps 
  $H_0 \Rightarrow_{v_1,p_1} H_2 \Rightarrow_{v_2,p_2} \cdots
  \Rightarrow_{v_n,p_n} H_n$ is called a \textit{derivation}.
  A derivation is called \textit{creative} if $H_0$ and $rhs(p_i)$ are all 
  mutually disjoint. We write $H \Rightarrow_* H'$ if there exists a creative
  derivation from $H$ to $H'$.
\end{definition}

\begin{example}
  A derivation in the above grammar of the string graph with three node vertices:
  \cstikz{tikz/line_derive.tikz}
  where again we color the newly established edges in red.
\end{example}

\begin{definition}[Starting Graph \cite{graph_grammar_handbook}]
  We say that $sn(S,z) \in GR_{\Sigma,\Gamma}$ is a \textit{starting graph} if
  it has only one node given by $z$, its label is $S$, the graph has no edges 
  and no connection instructions.
\end{definition}

\begin{definition}[Graph Grammar Language \cite{graph_grammar_handbook}]
  The graph language induced by a graph grammar
  $G=(\Sigma,\Delta,\Gamma,\Omega,P,S)$ is given by
  $L(G) = \{[H]\ |\ H \in GR_{\Delta,\Omega} \text{ and } sn(S,z)
  \Rightarrow_* H \text{ for some } z\}$, where $[H]$ denotes the equivalence
  class of all graphs which are isomorphic to $H$.
\end{definition}

\begin{definition}[Confluence \cite{graph_grammar_handbook}]
  We say that a graph grammar $G=(\Sigma,\Delta,\Gamma,\Omega,P,S)$ is
  \textit{confluent} if the following holds for every graph $H \in GRE_{\Sigma,
  \Gamma}$:
  if $H \Rightarrow_{u_1,p_1} H_1 \Rightarrow_{u_2,p_2} H_{12}$ and
  $H \Rightarrow_{u_2,p_2} H_2 \Rightarrow_{u_1,p_1} H_{21}$ are creative
  derivations of $G$ with $u_1 \not = u_2$, then $H_{12} = H_{21}$.
\end{definition}

There are simple and easily decidable conditions for determining if an edNCE
grammar is confluent. The class of confluent edNCE grammars is denoted
C-edNCE. % or simply VR (vertex replacement).

\begin{definition}[LIN-edNCE grammar \cite{graph_grammar_handbook}]
  An edNCE grammar $G$ is \textit{linear}, or a LIN-edNCE grammar, if for
  every production $X \to (D,C)$, $D$ has at most one nonterminal node.
\end{definition}

At any given point, only one non-terminal can be replaced, so LIN-edNCE grammars are automatically confluent. Hence, they are a subclass of C-edNCE grammars.


==> intro.tex <==
% -*- root: main.tex -*-

\begin{figure}%{r}{0.4\textwidth}
  \centering
  \stikz[0.7]{tikz/string_diagram_to_graph.tikz}
  \caption{A string diagram, and its encoding as a string graph}\label{fig:string-diagram-encode}
\end{figure}
String diagrams are essentially directed graphs, but instead of edges they have a more flexible notion of \textit{wires}. Wires can be left open at one or both ends to form inputs and outputs to the diagram, or can be connected to themselves to form a circle. They have a formal semantics given by monoidal category theory~\cite{joyal_street}, and have found applications in many fields. For example: in models of concurrency, they give an elegant presentation of Petri nets with boundary~\cite{Sobocinski:2010aa}, in computational linguistics, they are used to compute compositional semantics for sentences~\cite{LambekvsLambek}, in control theory, they represent signal-flow diagrams~\cite{Baez2014a,Bonchi2015}, and in theoretical physics, they provide the formal language of categorical quantum mechanics~\cite{picturalism}. A \textit{string graph} encodes a string diagram as a typed, directed graph, by replacing the wires with chains of edges containing special dummy vertices called \textit{wire-vertices} (see Fig.~\ref{fig:string-diagram-encode}).
By contrast, the ``real'' vertices, labelled here $f, g$ and $h$ are called \textit{node-vertices}. String graphs---originally introduced under the name ``open graphs'' in~\cite{open_graphs1}---have the advantage that they are purely combinatoric (as opposed to geometric) objects. %, and can be transformed using double-pushout (DPO) rewriting.
Equational reasoning on string diagrams is done by replacing sub-diagrams. The presence of dummy vertices in string graphs allows this to be done with double-pushout (DPO) graph rewriting. For example, in:
\begin{equation}\label{eq:subst-example}
  \stikz[0.7]{sg-sub.tikz}
\end{equation}
the LHS (shown in green above) is replaced by the RHS (blue), using the common boundary (red). This type of rewriting for string graphs is implemented in the graphical proof assistant Quantomatic~\cite{quantomatic}.

Often, one wants to reason not just about single string graphs, but entire families of them. However, informal notions of graphs with repetition are ill-suited for automated tools. To address this problem, \textit{!-graphs} (pronounced ``bang-graphs'') were introduced in~\cite{DD1} and formalised for string graphs in~\cite{pattern_graphs}. The idea behind !-graphs is that certain marked subgraphs (along with their adjacent edges) can be repeated any number of times, in a manner somewhat analogous to the Kleene star. These marked subgraphs are called \textit{!-boxes}. For example:
\[  \left \llbracket \stikz[0.7]{bang_graph2.tikz} \right \rrbracket
  =
  \stikz[0.7]{bang_graph_semantics.tikz}
\]
The !-graph in the semantic brackets represents the depicted set of string
graphs.
More precisely, an instance of a !-graph is obtained by repeatedly applying of the two operations EXPAND and KILL on the !-graph:
\begin{equation}\label{eq:bbox-ops}
  \stikz[0.7]{bang_graph2.tikz}
  \quad \overset{\textrm{EXPAND}_b}{\longrightarrow} \quad
  \stikz[0.7]{bang_graph2-exp.tikz}
  \qquad\qquad\qquad
  \stikz[0.7]{bang_graph2.tikz}
  \quad \overset{\textrm{KILL}_b}{\longrightarrow} \quad
  \stikz[0.7]{bang_graph2-kill.tikz}
\end{equation}
until all !-boxes have been eliminated. The set of concrete graphs (i.e. those not containing any !-boxes) obtainable from a !-graph via these operations is called the \textit{language} of the !-graph.

We call the set of languages expressible by !-graphs \textbf{BG}. In this paper, we will compare the expressiveness of this language to context-free vertex replacement grammars. We will focus on confluent neighbourhood-controlled embedding grammars, with directions and edge-labels, i.e.~\textbf{C-edNCE} grammars~\cite{graph_grammar_handbook}.

In arbitrary !-graphs, the !-boxes are allowed to nest inside of each other, but also overlap. The latter can generate patently non-context-free behaviour. Thus, it is natural to consider a restricted set of languages, \textbf{BGTO} of \textit{!-graphs with trivial overlap}. In this paper, we will give an algorithm for producing a C-edNCE grammar that is furthermore \textit{linear} (LIN-edNCE) which reproduces the language of any !-graph with trivial overlap. We therefore show the relationship between graph languages illustrated in Fig.~\ref{fig:venn1}.

\begin{figure} %{r}{0.4\textwidth}
\centering
\stikz[0.8]{venn_diagram.tikz}
\caption{Relationship between \textbf{LIN-edNCE}, \textbf{BG} and
\textbf{BGTO}} \label{fig:venn1}
\end{figure}

